Attentive Contextual Carryover for Multi-Turn End-to-End Spoken Language Understanding

Recent years have seen significant advances in end-to-end (E2E) spoken language understanding (SLU) systems, which directly predict intents and slots from spoken audio. While dialogue history has been exploited to improve conventional text-based natural language understanding systems, current E2E SLU approaches have not yet incorporated such critical contextual signals in multi-turn and task-oriented dialogues. In this work, we propose a contextual E2E SLU model architecture that uses a multi-head attention mechanism over encoded previous utterances and dialogue acts (actions taken by the voice assistant) of a multi-turn dialogue. We detail alternative methods to integrate these contexts into the state-ofthe-art recurrent and transformer-based models. When applied to a large de-identified dataset of utterances collected by a voice assistant, our method reduces average word and semantic error rates by 10.8% and 12.6%, respectively. We also present results on a publicly available dataset and show that our method significantly improves performance over a noncontextual baseline

==> related_work.tex <==
% (para. 1 review s2i, and say that s2i does not consider context, which is the important for multi-turn)
% End-to-end spoken language understanding (E2E SLU) has recently gained popularity from speech recognition and natural language processing research communities.
Previous research on E2E SLU has explored the two major defining properties of E2E SLU: directly inferring semantics from speech features~\cite{radfar2020end, serdyuk2018towards,qian2017exploring}; and jointly optimize ASR and NLU model components via common features across tasks ~\cite{haghani2018audio, ghannay2018end}. Recent research also shows that joint model approach can outperforms the approach that directly infer semantics from speech features in intent classification ~\cite{rao2020speech} and slot filling ~\cite{rongali2020exploring}. 
However, none of these previous works have used contextual signals for E2E SLU.

Historically, contextual signals have been shown to significantly improve composition SLU systems~\cite{bhargava2013easy, xu2014contextual, chen2015leveraging, sun2016intelligent}. These works are built on traditional machine learning methods. For example, adding previous utterances as context signals to an SVM-HMM SLU system ~\cite{bhargava2013easy} helped resolve ambiguities that occurred in multi-turn dialog. More recent works have incorporated contextual information into deep learning SLU systems. For ASR, \cite{pundak2018deep} developed a Contextual-LAS (CLAS) to embed contextual phrases during training and summarizes the available context via an extra attention layer. However, there have been concerns about the quality of contextual phrases on the E2E ASR performance and its scalability~\cite{wu2020multistate}. For example, CLAS approach would fail if the contextual phases do not appear in the utterance transcripts. 
To address this issue, recent work proposed multi-hot encoding for incorporating contextual information via the speech encoder into an RNN transducer network (RNN-T) and demonstrated that RNN-T ASR models can effectively use contexts such as dialog state to improve speech recognition~\cite{wu2020multistate}. For NLU,~\cite{chen2016end} proposed an architecture using end-to-end memory networks to model previous utterances in multi-turn conversations.  
%and shown that encoding previous utterances with the memory networks can improve state-of-art performance on multi-turn conversations. 
More recent research has shown that encoding dialog acts with a feedforward network from prior dialogue history result in a faster and more generalizable model without any loss in accuracy when compared to using end-to-end memory networks to encode previous utterances~\cite{gupta2018efficient}. \cite{wang2019effective} encodes historical utterances using the Bidirectional Long Short Term Memory networks and ConceptNet to encode external knowledge, and construct knowledge attention over these contexts.  Our work builds on and extends ~\cite{gupta2018efficient} and ~\cite{wu2020multistate} by employing a multi-head attention mechanism for encoding context and integrating the context encoder to state-of-the-art E2E SLU.
